Contracting With a Reinforcement Learning Agent by Playing Trick or Treat

We study principal-agent problems where a farsighted agent takes costly actions in an MDP. The core challenge in these settings is that agent's actions are hidden to the principal, who can only observe their outcomes, namely state transitions and their associated rewards. Thus, the principal's goal is to devise a policy that incentives the agent to take actions leading to desirable outcomes. This is accomplished by committing to a payment scheme (a.k.a. contract) at each step, specifying a monetary transfer from the principal to the agent for every possible outcome. Interestingly, we show that Markovian policies are unfit in these settings, as they do not allow to achieve the optimal principal's utility and are constitutionally intractable. Thus, accounting for history in unavoidable, and this begets considerable additional challenges compared to standard MDPs. Nevertheless, we design an efficient algorithm to compute an optimal policy, leveraging a compact way of representing histories for this purpose. Unfortunately, the policy produced by such an algorithm cannot be readily implemented, as it is only approximately incentive compatible, meaning that the agent is incentivized to take the desired actions only approximately. To fix this, we design an efficient method to make such a policy incentive compatible, by only introducing a negligible loss in principal's utility. This method can be generally applied to any approximately-incentive-compatible policy, and it generalized a related approach that has already been discovered for classical principal-agent problems to more general settings in MDPs.

==> approximation_oracle.tex <==
%\section{Approximation oracle}\label{sec:approx_oracle}
%\begin{algorithm}[H]
%	\caption{\texttt{Approximation oracle}}\label{alg:approx_oracle}
%	\begin{algorithmic}[1]
%		\Require $h \in \mathcal{H}, s \in \sset, \delta \in \mathbb{R}, \iota \in \mathcal{D}_\delta, M: \sset \times \mathcal{D}_\delta \rightarrow \mathbb{R} \cup \{-\infty\}$.
%		\If{$\mathcal{R}^\delta_{h,s,\iota}(M)$ is feasible}
%			\State $(\alpha,p,\widetilde{q}) \gets $ Solution to $\mathcal{R}^\delta_{h,s,\iota}(M)$
%			\State $v \gets G^\delta_{h,s,M}(\alpha,p,\widetilde{q})$
%			\State $z(a,s') \gets \argmax_{\iota' \in \mathcal{D}^{M,s'}_\delta : |\iota'-q(a,s')|< \delta} M(s',\iota') $ \label{line:oracle_discretizaion}
%		\Else
%			\State $(\alpha,p,\widetilde{q}) \gets$ anything
%			\State $v \gets -\infty$
%		\EndIf
%		\State \textbf{Return} $(\alpha,p,\widetilde{q},v)$
%	\end{algorithmic}
%\end{algorithm}
%
%Algorithm~\ref{alg:approx_policy} requires an approximation oracle that solves a relaxed version of the problem $\mathcal{P}_{h,s,\iota}(M)$ while satisfying Definition~\ref{def:approx_oracle}.
%In this section we describe how to build such an oracle.
%In order to obtain an approximate solution for the problem $\mathcal{P}_{h,s,\iota}(M)$, we solve an approximated problem $\mathcal{R}^\delta_{h,s,\iota}(M)$.
%For the ease of notation, we introduce the set $\mathcal{D}^{M,s}_\delta \coloneqq \{\iota \in \mathcal{D}_\delta \mid M(s,\iota)>-\infty\}$.
%
%To define $\mathcal{R}^\delta_{h,s,\iota}(M)$, we write the future promises $z(a,s')$ as a discretization of linear combinations of the promises in $\mathcal{D}_\delta$.
%This is accomplished by introducing the function $\widetilde{q}: \A \times \sset \rightarrow \Delta(\mathcal{D}_\delta)$, and defining the (continuous) future promise $q(a,s')$ as:
%\begin{equation*}
%	\label{eq:q_from_q_tilde}
%	q(a,s') \coloneqq \sum_{\iota' \in \mathcal{D}^{M,s'}_\delta} \widetilde{q}(\iota'|a,s') \iota',
%\end{equation*}
%for every action $a \in \A$ and future state $s' \in \sset$.
%Furthermore, we define the set of consistent functions $\widetilde{q}$ as:
%\begin{equation*}
%	\mathcal{Q}^M_\delta \coloneqq \{\widetilde{q}: \A \times \sset \rightarrow \Delta(\mathcal{D}_\delta) \mid \widetilde{q}(\iota'|a,s')=0 \; \forall a \in \A, s' \in \sset, \iota' \in \mathcal{D}_\delta \setminus \mathcal{D}^{M,s'}_\delta\}.
%\end{equation*} 
%In other words, $\widetilde{q} \in \mathcal{Q}^M_\delta$ if and only if $\widetilde{q}(a,s') \in \Delta(\mathcal{D}^{M,s'}_\delta)$ for every $a \in \mathcal{A}$ and $s' \in \sset$.
%
%The actual future promise $z(a,s')$ is instead defined by taking the promise $\iota' \in \mathcal{D}^{M,s'}_\delta$ such that $|q(a,s')-z(a,s')|<\delta$ and with the largest value of $M(s',z(a,s'))$, formally:
%\begin{equation*}\label{eq:z_from_q}
%	z(a,s') = d^{M,s'}_\delta(q(a,s')) \coloneqq \argmax_{\iota' \in \mathcal{D}^{M,s'}_\delta : |\iota'-q(a,s')|< \delta} M(s',\iota').
%\end{equation*}
%Observe that if $q(a,\omega,s') \in \mathcal{D}^{M,s'}_\delta$, then $z(a,\omega,s')=q(a,\omega,s')$, while otherwise $z(a,\omega,s')$ is one of the two promises in $\mathcal{D}^{M,s'}_\delta$ that are nearest to $q(a,\omega,s')$.
%
%Given this definitions, we let the objective function of the problem $\mathcal{R}^\delta_{h,s,\iota}(M)$ be:
%\begin{equation*}
%	G^\delta_{h,s,M}(\alpha,p,\widetilde{q}) \coloneqq \sum_{a \in \A} \alpha_a \sum_{s' \in \sset} P_h(s'|s,a) \left(r^P_h(s,p^a,s') +y(a,s')\right),
%\end{equation*}
%where $y(a,s') \coloneqq \sum_{\iota' \in \mathcal{D}^{M,s'}_\delta} \widetilde{q}(\iota'|a,s')M(s',\iota')$.
%
%Now we can define the problem $\mathcal{R}^\delta_{h,s,\iota}(M)$ as:
%\begin{equation*}
%	\widehat{G}^\delta_{h,s,\iota}(M) \coloneqq \max_{\substack{\alpha \in \Delta(\A)\\ p \in \mathcal{B}^{|\A|}\\ \widetilde{q}:\A \times \sset \rightarrow \Delta(\mathcal{D}_\delta)}}
%	G^\delta_{h,s,M}(\alpha,p,\widetilde{q}) \quad \text{s.t.} \quad (\alpha, p, q) \in \Psi^{h,s}_{\iota,\delta} \text{ and } \widetilde{q} \in \mathcal{Q}^M_\delta,
%\end{equation*}
%where $q$ is computed according to Equation~\ref{eq:q_from_q_tilde}.
%
%Let us remark that the problem $\mathcal{P}_{h,s,\iota}(M)$ is defined optimizing over the functions $z: \A \times \sset \rightarrow \mathcal{D}_\delta$ with values in the set $\mathcal{D}_\delta$, as the table $M : \sset \times \mathcal{D}_\delta$ is not defined for a promise $\iota \notin \mathcal{D}_\delta$.
%However, the ``relaxed'' set $\Psi^{h,s}_{\iota,\lambda}$ includes also any function $q: \A \times \sset \rightarrow \mathbb{R}$ with real values.
%This means that a solution $(\alpha,p,\widetilde{q})$ of $\mathcal{R}^\delta_{h,s,\iota}(M)$ does not correspond directly to a relaxed solution $(\alpha,p,z)$ by taking $z=q$, since $q(a,s')$ can be any convex combination of the promises in $\mathcal{D}_\delta$, thus may not be in $\mathcal{D}_\delta$ itself.
%For this reason, at Line~\ref{line:oracle_discretizaion} Algorithm~\ref{alg:approx_oracle} approximates the value of the future promise $q(a,s')$ to a value $z(a,s') = d_\delta^{M,s'}(q(a,s'))$ in $\mathcal{D}_\delta$.
%Due to this further approximation, the solution $(\alpha,p,z)$ does not belong to $\Psi^{h,s}_{\iota,\delta}$, but to a set $\Psi^{h,s}_{\iota,\lambda}$ with a larger $\lambda>\delta$. 
%
%\begin{restatable}{lemma}{rPolyTime}
%	\label{lem:lp_poly_time}
%	The problem $\mathcal{R}^\delta_{h,s,\iota}(M)$ can be solved in time polynomial in $\nicefrac{1}{\delta}$ and the instance size.
%\end{restatable}
%
%\begin{restatable}{lemma}{approxOracle}
%	\label{lem:approx_orcale}
%	If Algorithm~\ref{alg:approx_oracle} is used as an approximate oracle $O^{h,s}_{\iota,\delta}$ during the entire execution of Algorithm~\ref{alg:approx_policy}, then it satisfies Definition~\ref{def:approx_oracle}.
%\end{restatable}



==> pkgs.tex <==
\usepackage[letterpaper,margin=1in]{geometry}
% \usepackage{fullpage}
\usepackage{amssymb}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors


\usepackage{tikz}
\usetikzlibrary{shapes,backgrounds,patterns,calc,arrows,arrows.meta}
\usepackage{chemfig}

\catcode`\_=11
\definearrow5{-x>}{%
    \CF_arrowshiftnodes{#3}%
    \CF_expafter{\draw[}\CF_arrowcurrentstyle](\CF_arrowstartnode)--(\CF_arrowendnode)%
        coordinate[midway,shift=(\CF_ifempty{#4}{225}{#4}+\CF_arrowcurrentangle:\CF_ifempty{#5}{5pt}{#5})](line@start)%
        coordinate[midway,shift=(\CF_ifempty{#4}{45}{#4}+\CF_arrowcurrentangle:\CF_ifempty{#5}{5pt}{#5})](line@end)%
        coordinate[midway,shift=(\CF_ifempty{#4}{135}{#4}+\CF_arrowcurrentangle:\CF_ifempty{#5}{5pt}{#5})](line@start@i)%
        coordinate[midway,shift=(\CF_ifempty{#4}{315}{#4}+\CF_arrowcurrentangle:\CF_ifempty{#5}{5pt}{#5})](line@end@i);
    \draw(line@start)--(line@end);%
    \draw(line@start@i)--(line@end@i);%
    \CF_arrowdisplaylabel{#1}{0.5}+\CF_arrowstartnode{#2}{0.5}-\CF_arrowendnode
}
\catcode`\_=8

\usepackage{pict2e,picture,graphicx}
\usepackage[overload]{empheq}
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{booktabs}
\usepackage{amsmath}
\usepackage{cases}
\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{thm-restate}
\usepackage{enumitem}
\usepackage[ruled]{algorithm2e} % For algorithms
\renewcommand{\algorithmcfname}{ALGORITHM}
\SetAlFnt{\small}
\SetAlCapFnt{\small}
\SetAlCapNameFnt{\small}
\SetAlCapHSkip{0pt}
\IncMargin{-\parindent}
\allowdisplaybreaks
\usepackage{xcolor}
\usepackage{nicefrac, xfrac}
\usepackage{xparse}
%\usepackage{leftindex}
\usepackage{hyperref}
\usepackage{natbib}
\usepackage{cleveref}
\usepackage{wrapfig}
\usepackage{bbm}
%\usepackage{mathabx}
\usepackage{yfonts}
\usepackage{nicefrac} 
\usepackage{multirow}
\usepackage{bm}
\usepackage{bbm}
\usepackage{subcaption}
%\usepackage[sc]{mathpazo}
%\usepackage{libertine}
% \usepackage{fourier}
% \usepackage{libertinust1math}
\usepackage[T1]{fontenc}


\hypersetup{
	colorlinks = true,
	linkcolor = royalBlue,
	citecolor = darkGreen,
	linktocpage = true,
	urlcolor = mgreen
}

\usepackage{comment}

\usepackage{colortbl}
\usepackage{cellspace}

==> promise_form_with_full_def.tex <==
\section{Promise-form policies}\label{sec:promise_form}
As observed in Section~\ref{sec:history_necessary}, Markovian policies are both suboptimal and computationally intractable.
%
Therefore, in this work, we focus on the problem of computing a history-dependent policy.
%
However, history-dependent policies pose a computational challenge, as representing them requires an exponential number of bits with respect to the time horizon $H$.
%
To address this issue, we employ a class of policies—called \emph{promise-form} policies—that can be efficiently represented and are guaranteed to perform as well as history-dependent ones.
%
In this section, we first formally define a \emph{promise-form} policy, and we show that there always exists a \emph{promise-form} policy that is both IC and provides the principal's with a cumulative expected utility equal to $\textnormal{OPT}$.\footnote{A similar class of policies has been previously adopted in Bayesian persuasion settings~\citep{bernasconi2024persuading}, providing effective results when the agent is farsighted.\alb{Questa non mi paice.}}
%
\subsection{Promise-form policies}
A promise-form policy is defined as a tuple $\sigma \coloneqq \{(I_h,J_h,\varphi_h,g_h)\}_{h \in \mathcal{H}}$, where:
%
\begin{itemize}
	\item $I_h : \mathcal{S} \rightarrow 2^{[0,H]}$ is a function specifying, for every state $s \in \mathcal{S}$, a finite set $I(s) \subseteq [0,H]$ of promises for step $h \in \mathcal{H}$.
	%
	We assume that $|I_1(s)|=1$ for every $s \in \mathcal{S}$ and we denote with $i(s)$ the single element belonging to $|I_1(s)|$.
	%
	For ease of notation, we set $I_{H+1}(s) \coloneqq \{0\}$ for every $s \in \mathcal{S}$, and we let $\mathcal{I} \coloneqq \bigcup_{h \in \mathcal{H}} \bigcup_{s \in \mathcal{S}} I_h(s)$.
	%
	%\item $J_h:\sset \times \mathcal{I} \times \mathcal{A} \rightarrow \mathcal{B}$ is a function defining, for every state $s \in \mathcal{S}$, promise $\iota \in I_h(s)$ and action $a \in \mathcal{A}$, a finite set $J_h(s,\iota,a) \subseteq \mathcal{B}$ of contracts that the policy can propose when recommending action $a$ in state $s$ at step $h$ with promise $\iota$.
	%We let $\mathcal{J} \coloneqq \bigcup_{h \in \mathcal{H}} \bigcup_{s \in \mathcal{S}} \bigcup_{\iota \in I_h(s)} \bigcup_{a \in \mathcal{A}} J_h(s,\iota,a)$.
	\item $J_h:\sset \times \mathcal{I} \times \mathcal{A} \rightarrow \mathcal{B}$ is a function defining, for every state $s \in \mathcal{S}$, promise $\iota \in I_h(s)$, and action $a \in \mathcal{A}$, a finite set $J_h(s,\iota,a) \subseteq \mathcal{P}$ of contracts that the principal can commit to when recommending action $a \in \mathcal{A} $ in state $s \in \mathcal{S}$ with promise $\iota \in \mathcal{I}$, at step $h  \in \mathcal{H}$.
	%
	Furthermore, we let $\mathcal{J} \coloneqq \bigcup_{h \in \mathcal{H}} \bigcup_{s \in \mathcal{S}} \bigcup_{\iota \in I_h(s)} \bigcup_{a \in \mathcal{A}} J_h(s,\iota,a)$.
	%
	%\item $\varphi_h : \mathcal{S} \times \mathcal{I} \rightarrow \Delta(\mathcal{J} \times \mathcal{A})$ is an action-strategy to be use at time step $h \in \mathcal{H}$, where $\varphi_h(p,a|s,\iota)$ is the probability of committing to contract $p \in \mathcal{B}$ and recommending action $a \in \mathcal{A}$ in state $s \in \mathcal{S}$ when the promise is $\iota \in \mathcal{I}_h(s)$.
	\item $\varphi_h : \mathcal{S} \times \mathcal{I} \rightarrow \Delta(\mathcal{J} \times \mathcal{A})$ %\bac{perchè non è $\Delta(\mathcal{B} \times \mathcal{A})$? Perchè $\mathcal{J}$ è finito}
	encodes the policy at step $h \in \mathcal{H}$, with $\varphi_h(p,a | s, \iota)$ denoting the probability with which the principal commits to contract $p \in J(s,\iota,a)$ and recommends action $a \in \mathcal{A}$, when in a state $s \in \mathcal{S}$ with promise $\iota \in \mathcal{I}_h(s)$.
	%
	%\item $g_h : \mathcal{S} \times \mathcal{I} \times \mathcal{J} \times \mathcal{A} \times \mathcal{S} \rightarrow \mathcal{I}$ is a promise function for step $h \in \mathcal{H}$, where $g_h(s,\iota,p,a,s') \in I_{h+1}(s')$ is the promise for step $h+1$ when at step $h$ the state is $s \in \mathcal{S}$ and the promise is $\iota \in I_h(s)$, the principal recommends action $a \in \mathcal{A}$, propose contract $p \in J_h(s,\iota,a)$ and transitions to state $s' \in \mathcal{S}$.
	\item $g_h : \mathcal{S} \times \mathcal{I} \times \mathcal{J} \times \mathcal{A} \times \mathcal{S} \rightarrow \mathcal{I}$ is a promise function for step $h \in \mathcal{H}$, with $g_h(s,\iota,p,a,s') \in \mathcal{I}_{h+1}(s')$ being the promise for step $h+1$ when, at step $h \in \mathcal{H}$: the state is $s \in \mathcal{S}$, the promise is $\iota \in \mathcal{I}_h(s)$, the principal recommends action $a \in \mathcal{A}$, they commit to contract $p \in \mathcal{J}_h(s,\iota,a)$, and the environment transitions to state $s' \in \mathcal{S}$.
\end{itemize}
%
In a \emph{promise-form} policy, when reaching a state $s \in \mathcal{S}$ at step $h \in \mathcal{H}$, the principal promises a value $\iota \in I_h(s)$ to the agent that represents how much the agent will gain by following the principal’s recommendations. 
%
Furthermore, at each time step $h \in \mathcal{H}$, we notice that the principal’s contract-recommendations depend only on the current promise and the current state through the function $\varphi_h$.
%
% This removes the dependency on the history in the principal’s contract-recommendations, which may require employing an exponential number of bits with respect to the time horizon $H$.
%
However, both the cardinality of the set of promises $\mathcal{I}$ and the cardinality of the set of recommended contracts $\mathcal{J}$ may, in principle, be particularly large, thus potentially requiring a large number of bits to represent a promise-form policy.
%
In the rest of the paper, we show how to sidestep this issues by working with ``sufficiently small'' sets of promises and recommended contracts.
%
%\bollo{Scrivere un po'}

\bac{questo lo metterei in una nota}\bollo{Sì, l'idea era spostare queste commenti in appendix}\bollo{Con un abuso di notazione, $g_h$ è una promessa qualsiasi (e.g. la più bassa) dello stato futuro quando questa è valutata con un contratto fuori da $J_h(s,\iota,a)$}
\bollo{Come per le policy, definire $\mathcal{X}_\sigma$ per fare sommatorie su insiemi finiti}

\alb{Non ho capito cosa mettereste in appendice.}

\bollo{In questo momento dal main paper manca la definizione di $\mathcal{X}_\sigma$ e l'estenzione per formalità di $g(.)$. In più potrebbe essere comodo definire $V^{\text{P},\sigma}$, anche se non è strettamente necesssario.}
\bollo{Per orà l'estenzione per formalità di $g(.)$ è in una footnote in appendix. $\mathcal{X}_\sigma$ l'ho definito nel main paper in una riga}


\subsection{Implementing a promise-form policy}
We now discuss how the principal can implement a promise-form policy $\sigma$.
%
Specifically, we show how the principal, given a promise-form policy $\sigma$, can provide the agent with a contract-recommendation pair at each step $h \in \mathcal{H}$ based on the current history $\tau_h$.
%
To do so, we introduce Algorithm~\ref{alg:implement}, which takes as input the promise-form policy $\sigma$ that the principal has committed to, the time step $h \in \mathcal{H}$, and the history up to that time step $\tau_h$.
%
Then, in order to determine the current promise $\iota \in I_h(s_h)$, Algorithm~\ref{alg:implement} recursively composes the functions $g_h$ for the preceding steps $h'<h$ using the components of history $\tau_h$ it receives as input (See Line~\ref{line:implement_compute_next_iota}).
%
Once Algorithm~\ref{alg:implement} has computed the current promise $\iota \in I_h(s_h)$, it returns the contract-recommendation pair sampled from the function $\varphi_h$ evaluated in the current promise $\iota$ and in the current states $s_h$.
%
%
%
\begin{wrapfigure}[10]{R}{0.50\textwidth}
	\vspace{-0.9cm}
	\begin{minipage}{0.50\textwidth}
\begin{algorithm}[H]
	\caption{\texttt{Implement promise-form}}\label{alg:implement}
	\begin{algorithmic}[1]
		\Require $h \in \mathcal{H}$, \Statex $\tau = (s_1,p_1,a_1, \dots, s_{h-1},p_{h-1},a_{h-1},s_h)$, \Statex $\sigma = \{(I_h,J_h,\varphi_h,g_h)\}_{h \in \mathcal{H}}$.
		\State $\iota \gets i(s_1)$ \Comment{$I_1(s_1)$ contains only $i(s_1)$}
		\ForAll{$h'=1,\dots,h-1$}
		\State $\iota \gets g_{h'}(s_{h'},\iota,p_{h'},a_{h'},s_{h'+1})$ \label{line:implement_compute_next_iota}
		\EndFor
		\State $(p,a) \sim \varphi_h(s_h,\iota)$
		\State \textbf{Return} $(p,a)$
	\end{algorithmic}
\end{algorithm}
\end{minipage}
\end{wrapfigure}

In the following, given a promise-form policy $\sigma$, we denote with $\pi^\sigma$ the policy induced by $\sigma$ by following the procedure described above.
%
Formally, for each step $h \in \mathcal{H}$ and history $\tau_h$, we let $\pi^\sigma(\cdot|\tau) \coloneqq \varphi(\cdot|s_h, \iota^\sigma_\tau )$, where $\iota^\sigma_\tau$ is the promise computed according to Algorithm~\ref{alg:implement}, given in input the history $\tau$ and the promise-form policy $\sigma$.
We also let $\mathcal{X_\sigma} \coloneqq \mathcal{X}_{\pi^\sigma}$.
%\bollo{Magari tutte le definizioni ed il lemma che seuguono li spostiamo in appendix, quì scriviamo solo che si possono ridefinire funzioni equialenti che prendono $s$ e $\iota$ al posto di $\tau$.}


We also show that, given a promise-form policy $\sigma$, the value and action-value functions of its corresponding history-dependent policy $\pi^\sigma$ can be computed from the components that define the promise-form policy itself.
%
Formally, given a promise-form policy $\sigma$, we define the principal/agent value function ${V_{h}}^{\textnormal{P/A},\sigma}$ as the function that, for each step $h \in \mathcal{H}$, state $s \in \mathcal{S}$ and promise $\iota \in I_{h}(s)$, recursively satisfies:
%We define the following functions depending on the promise-form policy $\sigma$ and we show that they are equivalent to the value functions of the policy $\pi$ implemented by $\sigma$ with the procedure described above. Formally, we have:
%\bollo{Da scrivere meglio}
\begin{equation*}
	{V_{h}}^{\textnormal{P /A},\sigma} (s,\iota) \coloneqq \sum_{(p,a) \in \mathcal{X}_{\sigma}} \varphi_h(p,a | s,\iota)  {Q_{h}}^{\textnormal{P/A},\sigma} (s,\iota,p,a),
\end{equation*}
%
where the principal and the agent action-value functions are recursively defined as follows:
%
\begin{equation*}
	{Q_{h}}^{\textnormal{P},\sigma}(s,\iota,p,a) \coloneqq \sum_{s' \in \sset}P_h(s'|s,a) \left( r^\text{P}_h(s,p,s') + Q_{h+1}^{\textnormal{P},\sigma}(s',g_h(s,\iota,p,a,s')) \right),
\end{equation*}
and,
\begin{equation*}
	\qagentpr_h(s,\iota,p,a) \coloneqq \sum_{s' \in \sset} P_h(s'|s,a) \left(r^\text{A}_h(s,p,a,s') + \vagentpr_{h+1}(s',g_h(s,\iota,p,a,s')) \right).
\end{equation*}
for each step $h \in \mathcal{H}$, state $s \in \mathcal{S}$, contract $p \in \mathcal{J}$, action $a \in \mathcal{A}$ and promise $\iota \in I_{h}(s)$.
%
%\begin{equation*}
%	\vagentpr_h (s,\iota) \coloneqq \sum_{(p,a) \in \mathcal{X}} \varphi_h(p,a | s,\iota) \qagentpr_h(s,\iota,p,a),
%\end{equation*}
%
%\bac{queste le metterei in appendice}
We also define the value and action-value functions of the agent in the case in which the agent does not follow the principal's recommendation as follows:
\begin{equation*}
	\vagentdevpr_h(s,\iota) \coloneqq \sum_{(p,a) \in \mathcal{X}_\sigma} \varphi(p,a|s,\iota) \qagentdevpr_h(s,\iota,p,a).
\end{equation*}
\begin{equation*}
%	\bac{Q(s,i)?}
	\qagentdevpr_h(s,\iota,p,a) \coloneqq \max_{\widehat{a} \in A} \sum_{s' \in \sset} P(s'|s,\widehat{a}) \left(r^\text{A}_h(s,p,\widehat{a},s') +\vagentdevpr_{h+1}(s',g_h(s,\iota,p,a,s')) \right).
\end{equation*}
%
%
\begin{restatable}{lemma}{promiseFunctionsEq}
	\label{lem:promise_functions_eq}
	Given a promise-form policy $\sigma =\{(I_h,J_h,\varphi_h,g_h)\}_{h \in \mathcal{H}}$ and the corresponding history-dependent policy $\pi$, for any step $h \in \mathcal{H}$, history $\tau$ ending in state $s$, action $a \in \mathcal{A}$ and contract $p \in \mathcal{B}$, the following holds:
	\begin{align*}
		\vprincipalpr_h (s,\iota^\sigma_\tau) &= \vprincipal_h (\tau), \quad
		\qprincipalpr_h(s,\iota^\sigma_\tau,p,a) = \qprincipal_h(\tau,p,a), \\
		\vagentpr_h (s,\iota^\sigma_\tau) &= \vagent_h (\tau), \quad
		\qagentpr_h(s,\iota^\sigma_\tau,p,a) = \qagent_h(\tau,p,a), \\
		\vagentdevpr_h (s,\iota^\sigma_\tau) &= \vagentdev_h (\tau), \quad
		\qagentdevpr_h(s,\iota^\sigma_\tau,p,a) = \qagentdev_h(\tau,p,a),
	\end{align*}
	where $\iota^\sigma_\tau$ is computed according to Algorithm~\ref{alg:implement}.
\end{restatable}

\subsection{Honesty}
%
We now introduce a subclass of promise-form policies in which the principal honestly (approximately) fulfils the promises made to the agent.
%
Formally, we have:
%
\begin{definition}[$\eta$-honesty]
	A promise-form policy $\sigma =\{(I_h,J_h,\varphi_h,g_h)\}_{h \in \mathcal{H}}$ is $\eta$-honest, with $\eta \ge 0$, if, for every step $h \in \mathcal{H}$, state $s \in \mathcal{S}$, and promise $\iota \in I_h(s)$, the following holds:
	\begin{equation*}
		\left| \sum_{(p,a) \in \mathcal{X}_{\sigma}} \varphi_h(p,a|s,\iota) \sum_{s' \in \sset} P_h(s'|s,a) \left(r^\textnormal{A}_h(s,p,a,s') +g_h(s,\iota,p,a,s') \right) -\iota \right| \le \eta.
	\end{equation*} 
\end{definition}
%
Intuitively, a $\eta$-honest policy ensures that at the last time step $H$, the difference between the promise and the actual agent's expected utility is at most $\eta>0$.
%
Thus, by employing a recursive argument, it is possible to show that if $\sigma$ is $\eta$-honest, then the difference between the actual agent's utility and the promised one increases by at most $\eta > 0$ at each previous time step, as stated in the following lemma.
%
\begin{restatable}{lemma}{honestyValue}\label{lem:honesty_value}
	Let $\sigma =\{(I_h,J_h,\varphi_h,g_h)\}_{h \in \mathcal{H}}$ be a $\eta$-honest promise-form policy.
	Then, for every step $h \in \mathcal{H}$ and state $s \in \mathcal{S}$ it holds that $\left|\vagentpr_h(s,\iota)-\iota \right| \le \eta(H-h+1)$ for every $\iota \in I_h(s)$.
\end{restatable}
%
%\begin{restatable}{lemma}{promisePersuasive}
%	\label{lem:promise_persuasive}
%	Let $\sigma =\{(I_h,\varphi_h,g_h)\}_{h \in \mathcal{H}}$ be a $\eta$-honest promise-form policy such that for every step $h \in \mathcal{H}$, state $s \in \mathcal{S}$, promise $\iota \in I_h(s)$, actions $a,\widetilde{a} \in \mathcal{A}$ and contract $p \in \mathcal{B}$ such that $\varphi_h(p,a|s,\iota)>0$, the following constraint holds:
%	\begin{equation}
%		\label{eq:promise_persuasive}
%		\begin{split} 
%			\sum_{s' \in \sset} &P_h(s'|s,a) \left(r^\text{A}_h(s,p,a,s') +g_h(s,\iota,a,s') \right) \ge \\
%			&\sum_{s' \in \sset} P_h(s'|s,\widehat{a}) \left(r^\text{A}_h(s,p,\widetilde{a},s') +\vagentdevpr_{h+1}(s',g_h(s,\iota,a,s')) \right).
%		\end{split}		
%	\end{equation}
%	Then $\sigma$ is $\eta H$-persuasive. 
%\end{restatable}
%
We also introduce a crucial lemma showing that if an $\eta$-honest promise-form policy satisfies a suitable a set of ``local''constraints, then such a policy is also approximately IC.
%
%\bac{nel lemma sotto torna B come set di contratti.. sec me fa confusione con $\mathcal{J}$, quale è meglio usare?} \bollo{Sì, è da agiornare con $p \in J(s,\iota,a)$. Anche nella definizione $\sigma=...$ mancano i $J$ un po' dappertutto, e nella $g(...)$ manca il contratto prima dell'azione}
\begin{restatable}{lemma}{localICConstr}
	\label{lem:local_ic_constr}
	Let $\sigma =\{(I_h,J_h,\varphi_h,g_h)\}_{h \in \mathcal{H}}$ be a $\eta$-honest promise-form policy such that for every step $h \in \mathcal{H}$, state $s \in \mathcal{S}$, promise $\iota \in I_h(s)$, actions $a,\widehat{a} \in \mathcal{A}$ and contract $p \in \mathcal{B}$ such that $\varphi_h(p,a|s,\iota)>0$, the following constraint holds:
	\begin{equation}
		\label{eq:local_ic_constr}
		\begin{split} 
			\sum_{s' \in \sset} &P_h(s'|s,a) \left(r^\textnormal{A}_h(s,p,a,s') +g_h(s,\iota,p,a,s') \right) \ge \\
			&\sum_{s' \in \sset} P_h(s'|s,\widehat{a}) \left(r^\textnormal{A}_h(s,p,\widehat{a},s') +g_h(s,\iota,p,a,s') \right).
		\end{split}	
	\end{equation}
	Then, $\sigma$ is $2\eta H^2$-IC. 
\end{restatable}
%
%Thanks to Equation~\ref{eq:local_ic_constr}, we can require a policy to be $\epsilon$-IC imposing only a local constraint, \emph{i.e.}, for every state $s \in \sset$ and time step $h \in \mathcal{H}$, Equation~\ref{eq:local_ic_constr} depends only the current promise $\iota$, the policy at time step $h$ ($I_h,\varphi_h,g_h$), but no element of future time steps.
Thanks to Equation~\ref{eq:local_ic_constr}, we can require a policy to be approximately IC by only imposing a local constraint.
%
Indeed, for every state $s \in \sset$ and time step $h \in \mathcal{H}$, Equation~\ref{eq:local_ic_constr} depends only on the current promise $\iota$ and the components that define the promise-form policy $\sigma$.
%
%Given the previous results, we can prove that promise-form policies are sufficient to find the optimum.
Finally, given the previous results, we can prove that promise-form policies represent a subclass of history-dependent policies that is powerful enough to find the optimum.
%
\begin{restatable}{theorem}{promisingOptimal}
	\label{th:promising_optimal}
	There always exists a honest IC promising-form policy that achieves a principal's expected cumulative reward of $\textnormal{OPT}$.
\end{restatable}

%\subsection{Promise-form policies}
%A promise-form policy is defined by a set $\sigma = \{(I_h,J_h,\varphi_h,q_h,g_h)\}_{h \in \mathcal{H}}$, where:
%\begin{itemize}
%	\item $I_h : \mathcal{S} \rightarrow 2^{[0,H]}$ is a function defining, for every state $s \in \mathcal{S}$, a finite set $I(s) \subseteq [0,H]$ of promises for time step $h \in \mathcal{H}$.
%	We require that $0 \in I_1(s)$ for every $s \in \mathcal{S}$, and for the ease of notation we set $I_{H+1}(s) \coloneqq \{0\}$ for every $s \in \mathcal{S}$, and we let $\mathcal{I} \coloneqq \bigcup_{h \in \mathcal{H}} \bigcup_{s \in \mathcal{S}} I_h(s)$.
%	\item $J_h : \mathcal{S} \rightarrow 2^{[0,H]}$ is a function defining, for every state $s \in \mathcal{S}$, a finite set $J(s) \subseteq [0,H]$ of action-promises for time step $h \in \mathcal{H}$.
%	AS we did for $I_h(s)$ we require that $0 \in J_1(s)$ for every $s \in \mathcal{S}$, and for the ease of notation we set $J_{H+1}(s) \coloneqq \{0\}$ for every $s \in \mathcal{S}$, and we let $\mathcal{J} \coloneqq \bigcup_{h \in \mathcal{H}} \bigcup_{s \in \mathcal{S}} J_h(s)$
%	\item $\varphi_h : \mathcal{S} \times \mathcal{I} \rightarrow \Delta(\mathcal{X})$ is an action-strategy to be use at time step $h \in \mathcal{H}$, where $\varphi_h(p,a|s,\iota)$ is the probability of committing to contract $p \in \mathcal{B}$ and recommending action $a \in \mathcal{A}$ in state $s \in \mathcal{S}$ when the promise is $\iota \in \mathcal{I}_h(s)$.
%	\item $q_h : \mathcal{S} \times \mathcal{I} \times \A \rightarrow \mathcal{J}$ is an action-promise function for step $h \in \mathcal{H}$, where $q_h(s,\iota,a) \in J_h(s)$ indicates a refined action-promise when the current state is $s \in \mathcal{S}$, the current promise is $\iota \in I_h(s)$, and the principal has recommended action $a \in \S$.
%	The function $g_h$ must satisfy the following constraint:
%	\begin{equation*}
%		\label{eq:action_promise_constraint}
%		\sum_{(p,a) \in \mathcal{X}} q_h(s,\iota,a) \varphi_h(p,a|s,\iota) = \iota
%	\end{equation*}
%	for every step $h \in \mathcal{H}$, state $s \in \mathcal{S}$, and promise $\iota \in I_h(s)$. 
%	\item $g_h : \mathcal{S} \times \mathcal{A} \times \Omega \times \mathcal{I} \times \mathcal{S}$ is a promise function for step $h \in \mathcal{H}$, where $g_h(s,a,\omega,\iota,s') \in I_{h+1}(s')$ is the promise for step $h+1$ when at step $h$ the state is $s \in \mathcal{S}$ and the promise is $\iota \in I_h(s)$, the principal recommends action $a \in \mathcal{A}$ and transitions to state $s' \in \mathcal{S}$ through outcome $\omega \in \Omega$.
%\end{itemize}
%\bollo{Scrivere un po'}
%Intuitively, following a promise-form policy, when reaching a state $s \in \mathcal{S}$ at step $h \in \mathcal{H}$ the principal promises a cumulative reward $\iota \in I_h(s)$ to the agent.
%Such a promise represents a lower bound on the expected cumulative reward of the agent if they follow the recommendations from step $h$ onward.
%The function $\varphi_h$ is employed to choose randomly the current contract and action recommendation, while the function $g_h$ computes the next promise.
%The current promise $\iota$ is in expectation over the possible couples contract-action that the principal may recommend at step $h$.
%Since the agent can choose to deviate after the principal selects the current contract, the promise-form policy $\sigma$ includes a function $q_h$ to compute the promise given the selected contract.
%
%\subsection{Implementing a promise-form policy}
%
%\begin{algorithm}[H]
%	\caption{\texttt{Implement promise-form}}\label{alg:implement}
%	\begin{algorithmic}[1]
%		\Require $h \in \mathcal{H}, \tau = (s_1,a_1,\omega_1, \dots, s_{h-1},a_{h-1},\omega_{h-1},s_h), \sigma = \{(I_h,J_h,\varphi_h,q_h,g_h)\}_{h \in \mathcal{H}}$.
%		\State $\iota \gets 0$.
%		\ForAll{$h'=1,\dots,h-1$}
%			\State $\iota \gets g_{h'}(s_{h'},a_{h'},\omega_{h'},\iota,s_{h'+1})$
%		\EndFor
%		\State $(a,p) \sim \varphi_h(s_h,\iota)$
%		\State \textbf{Return} $(a,p)$
%	\end{algorithmic}
%\end{algorithm}
%
%We will denote with $\iota^\sigma_\tau$ the promise computed according to Algorithm~\ref{alg:implement}, given in input the history $\tau$ and the promise-form policy $\sigma$.
%
%We also show that the value and action-value functions of the principal and of the agent can be efficiently computed from the promise-form policy.
%We define the following functions depending on the promise-form policy $\sigma$ and show that they are equivalent to the value functions of the policy $\pi$ associated with $\sigma$.
%\bollo{Da scrivere meglio}
%\begin{equation*}
%	\vprincipalpr_h (s,\iota) \coloneqq \sum_{(p,a) \in \mathcal{X}} \varphi_h(p,a | s,\iota)  \qprincipalpr_h(s,\iota,p,a),
%\end{equation*}
%\begin{equation*}
%	\qprincipalpr_h(s,\iota,p,a) \coloneqq \sum_{\omega \in \Omega}F_h(\omega|s,a) \left( r^\text{P}_h(s,\omega,p) + \sum_{s' \in \sset} P_h(s'|s,w)\vprincipalpr_{h+1}(s',g_h(s,a,\omega,\iota,s')) \right).
%\end{equation*}
%
%\begin{equation*}
%	\vagentpr_h (s,\iota) \coloneqq \sum_{(p,a) \in \mathcal{X}} \varphi_h(p,a | s,\iota) \qagentpr_h(s,\iota,p,a),
%\end{equation*}
%\begin{equation*}
%	\qagentpr_h(s,\iota,p,a) \coloneqq \sum_{\omega \in \Omega}F_h(\omega|s,a) \left(r^\text{A}_h(s,\omega,p,a) + \sum_{s' \in \sset} P_h(s'|s,w)\vagentpr_{h+1}(s', g_h(s,a,\omega,\iota,s')) \right).
%\end{equation*}
%
%We also define the value and action-value functions of the agent in the case in which the agent does not follow the principal's recommendation as follows:
%\begin{equation*}
%	\vagentdevpr_h(s,\iota) \coloneqq \sum_{(p,a) \in \mathcal{X}} \varphi(p,a|s,\iota) \qagentdevpr_h(s,\iota,p,a).
%\end{equation*}
%\begin{equation*}
%	\qagentdevpr_h(s,\iota,p,a) \coloneqq \max_{\widehat{a} \in A} \sum_{\omega \in \Omega}F_h(\omega|s,\widehat{a}) \left(r^\text{A}_h(s,\omega,p,\widehat{a}) + \sum_{s' \in \sset} P(s'|s,\omega) \vagentdevpr_{h+1}(s',g_h(s,a,\omega,\iota,s')) \right).
%\end{equation*}
%
%\begin{restatable}{lemma}{promiseFunctionsEq}
%	\label{lem:promise_functions_eq}
%	Given a promise-form policy $\sigma =\{(I_h,J_h\varphi_h,q_h,g_h)\}_{h \in \mathcal{H}}$ and the corresponding history-dependent policy $\pi$, for any step $h \in \mathcal{H}$, history $\tau$ ending in state $s$, action $a \in \mathcal{A}$ and contract $p \in \mathcal{B}$, the following holds:
%	\begin{align*}
%		\vprincipalpr_h (s,\iota^\sigma_\tau) &= \vprincipal_h (\tau), \quad
%		\qprincipalpr_h(s,\iota^\sigma_\tau,p,a) = \qprincipal_h(\tau,p,a), \\
%		\vagentpr_h (s,\iota^\sigma_\tau) &= \vagent_h (\tau), \quad
%		\qagentpr_h(s,\iota^\sigma_\tau,p,a) = \qagent_h(\tau,p,a), \\
%		\vagentdevpr_h (s,\iota^\sigma_\tau) &= \vagentdev_h (\tau), \quad
%		\qagentdevpr_h(s,\iota^\sigma_\tau,p,a) = \qagentdev_h(\tau,p,a), \\
%	\end{align*}
%	where $\iota^\sigma_\tau$ is computed according to Algorithm~\ref{alg:implement}.
%\end{restatable}
%
%\subsection{Honesty}
%\begin{definition}[$\eta$-honesty]
%	A promise-form policy $\sigma =\{(I_h,J_h\varphi_h,q_h,g_h)\}_{h \in \mathcal{H}}$ is $\eta$-honest, with $\eta>0$, if, for every step $h \in \mathcal{H}$, state $s \in \mathcal{S}$, promise $\iota \in I_h(s)$, contract and action $(p,a) \in \mathcal{X}$ such that $\varphi_h(p,a|s,\iota)>0$ the following holds:
%	\begin{equation*}
%		\sum_{\omega \in \Omega}F_h(\omega|s,a) \left(r^\text{A}_h(s,\omega,p,a) + \sum_{s' \in \sset} P_h(s'|s,w)g_h(s,a,\omega,\iota,s') \right) \ge q_h(s,a,\iota) - \eta.
%	\end{equation*} 
%\end{definition}
%
%\begin{restatable}{lemma}{honestyValue}
%	\label{lem:honesty_value}
%	Let $\sigma =\{(I_h,J_h\varphi_h,q_h,g_h)\}_{h \in \mathcal{H}}$ be a $\eta$-honest promise-form policy.
%	Then, for every step $h \in \mathcal{H}$ and state $s \in \mathcal{S}$ it holds that $\vagentpr_h(s,\iota) \ge \iota - \eta(H-h+1)$ for all $\iota \in I_h(s)$.
%\end{restatable}
%
%\begin{restatable}{lemma}{promisePersuasive}
%	\label{lem:promise_persuasive}
%	Let $\sigma =\{(I_h,J_h\varphi_h,q_h,g_h)\}_{h \in \mathcal{H}}$ be a $\eta$-honest promise-form policy such that for every step $h \in \mathcal{H}$, state $s \in \mathcal{S}$, promise $\iota \in I_h(s)$, actions $a,\widetilde{a} \in \mathcal{A}$ and contract $p \in \mathcal{B}$ such that $\varphi_h(p,a|s,\iota)>0$, the following constraint holds:
%	\begin{equation}
%	\label{eq:promise_persuasive}
%	\begin{split} 
%		\sum_{\omega \in \Omega}&F_h(\omega|s,a) \left(r^\text{A}_h(s,\omega,p,a) + \sum_{s' \in \sset} P_h(s'|s,w)g_h(s,a,\omega,\iota,s') \right) \ge\\
%		&\sum_{\omega \in \Omega}F_h(\omega|s,\widehat{a}) \left(r^\text{A}_h(s,\omega,p,\widehat{a}) + \sum_{s' \in \sset} P_h(s'|s,w)\vagentdevpr_{h+1}(s',g_h(s,a,\omega,\iota,s')) \right).
%	\end{split}		
%	\end{equation}
%	Then $\sigma$ is $\eta H$-persuasive. 
%\end{restatable}
%
%\begin{restatable}{theorem}{promisingOptimal}
%	There always exists a promising-form policy that achieves a principal's expected cumulative reward of $\text{OPT}$.
%\end{restatable}

